Search for diboson resonances with boson-tagged jets in $pp$ collisions at $\sqrt{s}=13$ TeV with the ATLAS detector

Narrow resonances decaying into $WW$, $WZ$ or $ZZ$ boson pairs are searched for in 36.7 fb $^{-1}$ of proton-proton collision data at a centre-of-mass energy of $\sqrt{s}=13$ TeV recorded with the ATLAS detector at the Large Hadron Collider in 2015 and 2016. The diboson system is reconstructed using pairs of large-radius jets with high transverse momentum and tagged as compatible with the hadronic decay of high-momentum $W$ or $Z$ bosons, using jet mass and substructure properties. The search is sensitive to diboson resonances with masses in the range 1.2-5.0 TeV. No significant excess is observed in any signal region. Exclusion limits are set at the 95% confidence level on the production cross section times branching ratio to dibosons for a range of theories beyond the Standard Model. Model-dependent lower limits on the mass of new gauge bosons are set, with the highest limit set at 3.5 TeV in the context of mass-degenerate resonances that couple predominantly to bosons.

==> Sections/EventSelection.tex <==
%-------------------------------------------------------------------------------%
% Description of the event selection cuts
%-------------------------------------------------------------------------------%

\section{Event Selection}
\label{sec:eventselection}

